Diversity Analysis of Millimeter-Wave OFDM Massive MIMO Systems

We analyze the diversity gain for a distributed antenna subarray employing orthogonal frequency-division multiplexing (OFDM) in millimeter-wave (mm-Wave) massive multiple-input multiple-output (MIMO) systems. We show that the diversity gain depends on the number of transmitted data streams, the number of remote antenna units, and the number of propagation paths between RAUs. Furthermore, we show that by using bit-interleaved coded multiple beamforming (BICMB), one can achieve the maximum diversity gain in a distributed antenna subarray system. The assumption in both scenarios is that the number of the antennas at the transmitter and the receiver are large enough and channel state information (CSI) is known at the transmitter and the receiver.

==> diversity_general.tex <==
\section{Diversity Gain and PEP Analaysis for more general case} \label{bicmb_ofdm_diversity_general}

Unlike the previous section, where the assumption was that each subcarrier should be used at least once, i.e., each element of $\bm{\alpha}$ is nonzero, in this section we study the case where the use of each subchannel can be zero as well. 

We consider a similar system to the one in Fig. \ref{fig::bicmb_ofdm_model}. Similar to \cite{Li2013}, we find an uppernound for the PEP. By using (\ref{eq::bicmb_ofdm_su_PEP1}), and defining matrix $\mathbf{A}$ such that the $k$th row of this matrix represents the $k$th subcarrier.

One can see that each channel tap is statisically independent and can be written as 
\begin{align}
E\left[h_{m,n}(l)h_{m,n}^*(l) \right] =  \left\{ 
	\begin{array}{ll}
		0  &   l\neq l' \\
		\frac{1}{L} & l=l',
	\end{array}
	\right. 
\end{align}
where $ h_{n,n}(l) $ denotes the $(m,n)$th element of $\mathbf{H}(l)$ and is given as
\begin{align}
	h_{n,n}(l) = \frac{1} {\sqrt{L} } \alpha_{i,j}^l \exp \left[  j\frac{2\pi d}{\lambda} \left((m-1)\sin\phi_{i,j}^l - (n-1)\sin\theta_{i,j}^l\right)\right].
\end{align} 
%

One can define 

\begin{align}
\rho &= \frac{E\left[\tilde{h}_{m,n}(k)\tilde{h}_{m,n}^*(k')\right]} {\sqrt{  E\left[\tilde{h}_{m,n}(k)\tilde{h}_{m,n}^*(k)\right] E\left[\tilde{h}_{m,n}(k') \tilde{h}_{m,n}^*(k')\right]    }} \nonumber  \\
& = \left|\frac{\sum_{l=1}^{L}  \exp\left( -j\frac{2\pi(k-k')\tau_{i,j}^{l} }{KT_s}\right)  E\left[h_{m,n}(l)h_{m,n}^*(l) \right]  }{E\left[h_{m,n}(l)h_{m,n}^*(l) \right]}\right| \nonumber \\
& = \frac{1}{L} \left| \sum_{l=1}^{L} \exp\left[-j\frac{2\pi(k-k')\tau_{i,j}^{l} }  {KT_s}\right] \right| \nonumber \\
& = \frac{1}{L} \left|   \frac{1-\exp\left[-j\frac{2\pi(k-k')\tau_{i,j}^l}{KT_s}\right]} {den}   \right |
	\end{align}
	
		% 
